CONQRR: Conversational Query Rewriting for Retrieval with Reinforcement Learning

Compared to standard retrieval tasks, passage retrieval for conversational question answering (CQA) poses new challenges in understanding the current user question, as each question needs to be interpreted within the dialogue context. Moreover, it can be expensive to re-train well-established retrievers such as search engines that are originally developed for non-conversational queries. To facilitate their use, we develop a query rewriting model CONQRR that rewrites a conversational question in the context into a standalone question. It is trained with a novel reward function to directly optimize towards retrieval using reinforcement learning and can be adapted to any off-the-shelf retriever. CONQRR achieves state-of-the-art results on a recent open-domain CQA dataset containing conversations from three different sources, and is effective for two different off-the-shelf retrievers. Our extensive analysis also shows the robustness of CONQRR to out-of-domain dialogues as well as to zero query rewriting supervision.

==> tables/DE_versus_BM25_rewrite.tex <==
\begin{table*}%[h]
\centering
\small
\begin{tabular}{p{3.3cm}|p{11.7cm}}
\toprule
Dialogue Context & \textit{Q}: When did Steve McQueen star in Ford Commercials? \newline
\textit{A}: In 1998 director Paul Street created a commercial \dots \newline
\dots \newline
\textit{A}: In 2005, Ford used Steve McQueen's likeness again \dots \newline
\textit{A}: What was noteworthy about these Ford commercials? \\
\midrule
\ours (mix) w/ BM25 & What was noteworthy about the Ford commercials Steve McQueen did in 2005? (BM25 Rank=1)  \\
\ours (mix) w/ DE & What was noteworthy about the Ford commercials starring Steve McQueen? (DE Rank=6) \\
T5QR & What was noteworthy about the Ford commercials? (BM25 / DE Rank >100) \\
\bottomrule
\end{tabular}
%\end{adjustbox}
\caption{Examples of rewrites from \ours trained with rewards from different retrievers, as well as T5QR. \label{tab:de_vs_bm25}}
\end{table*}

==> tables/sl_versus_rl.tex <==
\begin{table*}%[!htp]
\centering
\small
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{llccc|ccc|cccc}\toprule
\multirow{3}{*}{\textbf{QR Model}}
&\multirow{3}{*}{\textbf{IR System}} &\multicolumn{3}{c}{\textbf{QuAC-Conv}}
&\multicolumn{3}{c}{\textbf{NQ-Conv}} &\multicolumn{3}{c}{\textbf{TREC-Conv}}\\
&&MRR &R@10 &R@100 &MRR &R@10 &R@100 &MRR &R@10 &R@100 \\\midrule
T5QR & BM25  & 0.33 & 52.7 & 85.0 & 0.345 & 54.2 & 83.9 & 0.230 & 44.5 & 82.3 \\
\ours (mix) & BM25  & 0.379 & 59.2 & 90.9 & 0.385 & 58.8 & 88.9 & 0.229 & 44.7 & 82.7 \\
\ours (RL) & BM25  &  & & & & & & & & \\
Human & BM25  & 0.403 & 62.9 & 98.4 & 0.408 & 63.8 & 99.0 & 0.273 & 53.8 & 98.9 \\\midrule
T5QR & BM25-light & 0.292 & 46.0 & 69.8 & 0.367 & 53.7 & 77.2 & 0.254 & 46.2 & 74.7 \\
\ours (mix) & BM25-light & 0.344 & 53.6 & 77.4 & 0.408 & 58.3 & 82.4 & 0.270 & 49.6 & 76.1 \\
\ours (RL) & BM25-light & & & & & & & & & \\
Human & BM25-light & 0.363 & 55.8 & 79.7 & 0.445 & 63.0 & 86.7 & 0.315 & 57.2 & 85.4 \\\midrule
T5QR & DE & 0.349 & 55.7 & 76.1 & 0.417 & 58.7 & 74.2 & 0.343 & 55.9 & 79.2 \\
\ours (mix) & DE & 0.387 & 62.0 & 82.4 & 0.439 & 62.2 & 79.0 & 0.361 & 58.9 & 81.0 \\
\ours (RL) & DE & 0.416 & 65.9 & 85.8 & 0.453 & 64.1 & 80.9 & 0.327 & 55.2 & 79.6 \\
Human & DE & 0.409 & 64.5 & 84.1 & 0.483 & 65.8 & 83.2 & 0.411 & 66.0 & 86.5 \\
\bottomrule
\end{tabular}
}
\caption{SL versus RL.}
\label{tab:sl_vs_rl}
\end{table*}
